Weakly Supervised Named Entity Tagging with Learnable Logical Rules

We study the problem of building entity tagging systems by using a few rules as weak supervision. Previous methods mostly focus on disambiguation entity types based on contexts and expert-provided rules, while assuming entity spans are given. In this work, we propose a novel method TALLOR that bootstraps high-quality logical rules to train a neural tagger in a fully automated manner. Specifically, we introduce compound rules that are composed from simple rules to increase the precision of boundary detection and generate more diverse pseudo labels. We further design a dynamic label selection strategy to ensure pseudo label quality and therefore avoid overfitting the neural tagger. Experiments on three datasets demonstrate that our method outperforms other weakly supervised methods and even rivals a state-of-the-art distantly supervised tagger with a lexicon of over 2,000 terms when starting from only 20 simple rules. Our method can serve as a tool for rapidly building taggers in emerging domains and tasks. Case studies show that learned rules can potentially explain the predicted entities.

==> 1-intro-v2.tex <==

%
% 1 background, supervised methods require manual labels 
%    distantly supervised method requires knowledge bases
%    domain-heuristics require domain expertise, 


%
% 2 studies the problem under minimal supervision setting, which is still a challenging problem (Claire Cardie), without manual labels, effort, example domains.

% 3 motivation, intuition, logical rules can be used to recognize entities, 
%  ==== solve 2 problems
%      ---(a) boundary detection
%      -- (b) semantic drift 
%    logical rules can be learned from unlabeled data: example and explanation 
% 4 framework, span based NER, overview,  
%  * logical rules, compound rules
%  * how to induce new rules 
%  * 

% Named entity recognition is an important component of many downstream information extraction tasks (e.g.~relation extraction) and knowledge base construction.
 % \cite{example-related-RelationExtraction-EventExtraction-work-using-NER, and knowledge-base-construciton}.(\todo{add refs} )
% Different classes of approach have been proposed for entity recognition; 

% Supervised NER models~\cite{Ma2016EndtoendSL,Lample2016NeuralAF} have achieved 
% reliable performance due to advances in 
% neural models and the availability of manual annotation.  
% However, manually obtaining a large amount of labeled data is often a bottleneck for supervised methods.

Training accurate supervised NER models~\cite{Ma2016EndtoendSL,Lample2016NeuralAF} requires many manual annotations, which is a bottleneck to apply them to new domains and tasks. 
Distantly supervised approaches~\cite{Ren2015ClusTypeEE, He2017AutoentityAE, Shang2018LearningNE, Peng2019DistantlySN} 
alleviate this problem by using 
%have been proposed to build NER models with 
manually constructed lexicons or knowledge bases. 
But, as we show in our experiments, the performance of these methods is highly dependent on the size and accuracy of lexicons, and is dramatically worse with small or automatically learned lexicons. 
Studying weakly supervised NER methods that can automatically learn more rules from a few seed rules is desirable because 
(1) rules are effective, interpretable, and can be used to ``debug'' prediction errors; 
(2) developed methods can be rapidly deployed to new domains or types of entities with significant less manual effort.



\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{Figures/fig-example-v4-small.pdf}
% 	\vspace{-1mm}
    \caption{
    Examples of a seed logical rule and a newly induced rule from labeled data for recognizing locations. `x' denotes a token span from a given sentence. 
    }
    \label{fig:logicalrule}
    \vspace{-4mm}
\end{figure}
Weakly supervised methods such as SwellShark~\cite{Fries2017SwellSharkAG}, Snorkel~\cite{Ratner2017SnorkelRT} adopt two-stage pipeline that annotates data by manual rules and then trains machine learning models on labeled data. Bootstrapping frameworks~\cite{Huang2010InducingDS, niu2003bootstrapping, Gupta2014ImprovedPL} recognize entities in corpus by iterations. However,
these methods focus on learning how to classify entity types and assume that entity boundaries are given by syntax analysis (e.g., POS tags) and have perfect recall.
%convert structured prediction tasks like sequence tagging to classification by first generating candidate spans from the sequence and independently labeling each candidate. These methods assume candidate spans have perfect recall. 
Unfortunately, syntax based boundary detection cannot cover entity boundaries well.
%because generating candidate spans heavily relies on noun phrases by dependency parsing, 
 As shown in Table~\ref{tab:bound_detection}, we test the performance of noun phrases from syntax analysis on three datasets and find that noun phrases can only cover $50\%$ of entity boundaries in BC5CDR and CONLL2003, and $35\%$ in CHEMDNER. If these frameworks fail to identify a span boundary correctly, there is no way for them to recover from the mistake. To improve entity boundary detection, SwellShark~\cite{Fries2017SwellSharkAG} uses both noun phrases and an expert-made candidate generator.
\citet{Safranchik2020WeaklySS, Lison2020NamedER} allow users to write heuristic rules to detect boundaries and assign types at the same time. 
%These methods allow users to provide a dictionary or rules as supervision. 
However, it is often challenging and impractical for people to 
%come up with an 
produce an
accurate and complete set of labeling rules or candidate generator, requiring both a significant amount of time and domain expertise. Hence, it is still challenging for existing methods to detect entity boundaries under minimal supervision.
\begin{table}[t]
    \center
    \small
    \begin{tabular}{r|ccc|ccc}
        \toprule
                & \multicolumn{3}{c}{Noun phrase}  & \multicolumn{3}{c}{Our method} \\
                    
        \cmidrule{2-7}
             &  P & R & F$_1$ & P & R & F$_1$ \\
        \midrule
        
        BC5CDR & 17.1 & 50.1 & 25.5 & 69.8 & 67.8 & 68.7\\
        CHEM & 3.2 & 35.6 & 5.8 & 63.0 & 60.2 & 61.6\\
        CoNLL & 4.1 & 47.3 & 7.5 & 86.9 & 86.7 & 86.8\\
        
        \bottomrule
    \end{tabular}
    \caption{
   Boundary detection performance from our method and parsing based noun phrases.
  }
    \label{tab:bound_detection}
%}
    \vspace{-4mm}
    \end{table}

% To obtain 
% %boundary of entities, 
% entity boundaries,
% previous works have 
% %three ways: 
% explored three techniques:
% (1) Noun phrases from dependency parsing; (2) Accurate and complete rules; (3) Large lexicons. However, complete rules and large lexicons need a large amount of human effort with in-domain knowledge;
% %and these efforts 
% such effort
% can be even 
% %harder 
% more expensive
% than dataset annotation. Noun phrases cannot provide accurate 
% %information of boundary 
% boundary information
%for NER tasks as we show in Table~\ref{tab:bound_detection}. Hence, 
In this paper, to further reduce human efforts we propose a NER system that is able to automatically learn rules and lexicons from datasets starting from only a small set of seed rules. %What's more, 
Furthermore,
these learned rules 
%cannot only 
can both
assign categories and detect accurate span boundaries for NER.
Our work is motivated by the intuition that new logical rules can be learned from unlabeled data using a small set of seed rules. 
For example, given a seed rule (e.g.~if a token span is ``Dallas'', then it is a Location) as shown in Figure~\ref{fig:logicalrule}, 
we can induce a new rule (i.e.,~if a token span is a proper noun and its preceding tokens are ``lives in'', then it is a Location) from the instances labeled by the seed rule. Based on this intuition, we define five types of logical rule templates considering 
the lexical, local context, and syntax information of entities. 
We enumerate all spans up to a fixed length and extract spans that are matched by logical rules.
%From predefined rule templates, our model can learn a set of precise logical rules to improve NER performance.
%We focus on two key issues for learning accurate logical rules. First, 
We notice that simple logical rules are often inaccurate when detecting entity boundaries. 
For example, given the sentence ``{\it John lives in Dallas where he was born}'', the simple rule ``lives in \underline{~~}'', which is a preceding context clue, will match multiple token spans such as ``Dallas'', ``Dallas where'', ``Dallas where he'' etc. 
To detect entity boundaries accurately, we propose to use compound rules, which are formed from simple rules and logical connectives (e.g.~``and''). 
For example, using both the preceding context and the part-of-speech (POS) tag rule (e.g.~``lives in \underline{~~}'' and POS is a proper noun) can accurately identify the entity ``Dallas''. 

%Second, we observe that the semantics of learned logical rules will soon drift away from
Due to a large amount of enumerated spans and bias from a small set of seed rules, the learning process may induce many noisy instances and rules.
%To alleviate this problem, we propose to first train a neural network model using the instances labeled by seed rules. Then, we predict the labels of unlabeled data using the trained model and select new logical rules based on the predictions. 
To alleviate this problem, we adopt an embedding based instance selection mechanism which measures similarity between entities by embedding
%knowledge in embedding 
to maintain a precise entity set. The precise entity set enables our framework to maintain precision of recognized entities while increasing recall, as we show in our experiments.

% Specifically, our algorithm first collects high-quality weak labels by applying seed rules to unlabeled data and trains a neural NER model with these labels. 
% Since the coverage of seed rules is limited,
%  we expand the weak labels by predicting the labels of unlabeled data using the trained NER model. 
% Next, we score all candidate rules extracted from unlabeled data using the expanded weak labels. 
% Finally, we select and add 
% the
% top-scoring rules to 
% the
% seed rules for another iteration of learning.

%
%
%Next, we predict the labels of unlabeled data using the trained model and compute the confident scores of all candidate rules extracted from unlabeled data using the predicted labels. Then, we select and add top-scored rules to seed rules for another iteration learning. 
%
%We conduct experiments on three datasets and explore several rule selection strategies. 
Experimental results show that our method outperforms existing weakly supervised methods and can increase an average $F_1$ score by $60\%$
%$24$-point 
across three datasets over methods using only seed rules. User study shows that learned rules can easily explain the recognized entities including boundary and type to help users understand NER results. For example, given a sentence ``a patient with SAH and'', and rule ``a patient with \underline{~~} and'', we can easily understand why ``SAH'' is an entity and type is disease.


%To the best of our knowledge, our framework is the first to recognize and type entities from a small set of seed logical rules by considering both symbolic rules and neural representations of entities. 
%Jiacheng edits:
% We propose to recognize and type entities from a small set of seed logical rules. Our framework considers bother symbolic rules and neural representations of entities. 
% We propose a bootstrapping framework to learn logical rules for entity recognition. 
In summary, our main contributions are:
\begin{itemize}

    \item We propose to learn compound logical rules that can detect entity boundaries and classify types simultaneously. Learned rules can work as explanation which is still an open problem in NER task.
    %\item  We propose a method that can automatically learn a set of logical rules to further reduce supervision (i.e.,~lexicon, rules) required from humans. Learned rules can also work as explanations which is still an open problem in NER tasks. 
    %by considering both the information from seed rules and intrinsic entity similarities embedded in neural representations.
    
    \item To learn logical rules and reduce noise from rules, we propose a framework with a dynamic selection strategy to maintain a high-precision entity set during training.
    %\item  To detect entity boundaries, we define five types of simple logical rule templates and propose to label named entities using compound logical rules.
    
    \item  We conduct experiments on both general and domain-specific datasets to demonstrate the effectiveness of our method. 
    %We also conduct a user study concerning the explainability of learned logical rules. Our study shows that 79\% of test cases with logical rules can be used as understandable explanations.
    A user study shows that users can understand $79\%$ test cases by logical rules which proves the explainability of learned logical rules.
    %for the prediction.
    
    
%    \hb{0. define 5 types of logical rules that are very effective ??}
%    \hb{1. propose to learn compound logical rules that can detect entity boundaries and classify types simultaneously ?}
%    \hb{2. design a dynamic selection strategy for selection high-quality labels? }
%    \hb{3 conduct experiments on 3 datasets and demonstrate the effectiveness of our method. }
%    \hb{4 conduct user study to show that learned rules can be easily understood by users ??}
    
    
\end{itemize}


\begin{figure*}[t]
\centering
 \includegraphics[width=\textwidth]{Figures/fig-framework-v3.pdf}
\caption{
Overview of our bootstrapping framework with logical rules and examples for each step. 
}
\label{fig:overview}
\vspace{-4mm}
\end{figure*}

% =======Above are new version of intro ===

% ======




==> 1-introduction.tex <==
Named entity recognition 
is an important 
%task for 
component of
many downstream information extraction tasks (e.g.~relation extraction) and knowledge base construction. Supervised named entity recognition has achieved reliable performance due to advances in 
%deep 
neural models 
%without 
that circumvent the need for
handcrafted features~\cite{Ma2016EndtoendSL,Lample2016NeuralAF}. However, supervised models require a large amount of manual annotation for training. This is challenging in specific domains or low-resource languages, where domain-expert annotation is hard to obtain.

\begin{figure}[t]
	\centering
	%\includegraphics[width=0.49\textwidth]{Figures/Figure1.pdf}
	\includegraphics[width=\linewidth]{Figures/fig-example-v2-small.pdf}
% 	\vspace{-1mm}
    \caption{
    Example logical rule from BC5CDR dataset. Given a seed rule, our model selects new logical rules from a corpus and matches new entities.
    %\hb{Please share the picture link here!}
    }
    \label{fig:logicalrule}
    \vspace{-2mm}
\end{figure}

To reduce human effort, a few distantly supervised approaches~\cite{Ren2015ClusTypeEE, He2017AutoentityAE, Shang2018LearningNE, Peng2019DistantlySN} automatically generate labeled data from open knowledge bases or dictionaries. Distant supervision makes it possible to generate training data for NER at large scale without expensive 
%human efforts. 
labeling effort.
However, in many cases, an open knowledge base is not available (e.g.~technical documents). Another line of 
work
%reply on 
relies on
complicated rules from in-domain experts to replace hand-labeled 
%training 
data for training~\cite{Safranchik2020WeaklySS, Fries2017SwellSharkAG, Ratner2017SnorkelRT}. \citet{Fries2017SwellSharkAG} used an expert-made candidate generator to achieve similar performance with distantly supervised methods. \citet{Safranchik2020WeaklySS} incorporated multi-type rules including dictionaries and domain-specific rules. They proposed tagging rules and linking rules which incorporate both dictionaries and domain-specific rules. Although dictionaries and rules reduce human effort 
%on annotated 
to annotate
data, 
%dictionaries and rules 
they
are still not easy to obtain and usually need 
%a large amount of 
significant
in-domain 
expert
knowledge.
%from human.

Bootstrapping enables models to obtain large amounts of weakly-labeled data given 
%some 
a few
seeds. Bootstrapping is widely used for Entity Set Expansion (ESE)~\cite{Shen2017SetExpanCS, Yan2019LearningTB} which acquires new instances of a specific category by iteratively evaluating and selecting patterns, while extracting and scoring entities. 
Bootstrapping frameworks 
%is 
are
also applied on semantic class taggers~\cite{Huang2010InducingDS}, which assign a semantic class for each entity. 
\citet{Zhang2020BootstrappingNE} leverages dependency parsing rules (i.e.,~``compound'' relations) to recognize entities from text, but 
%only 
dependency parsing rules 
alone
cannot 
always
recognize entities precisely.
%in many cases. 
Hence, recognizing entities (i.e.,~boundary information) from plain text is still a challenging task for boostrapping.

Intuitively, a single rule usually cannot provides accurate 
%information for boundary. 
boundary information.
Considering the following example:

\begin{center}
    \texttt{The new company is called AdOn GmbH and is located in Hamburg.}
\end{center}

The Pre-Ngram rule $\texttt{company is called}\rule{0.4cm}{0.15mm}$ provides strong information for the start of an organization entity but the end of 
the
entity is 
lost.
%losing. 
However, we could 
%compose 
combine
a Post-Ngram rule $\rule{0.4cm}{0.15mm}\texttt{and is located}$ with the Pre-Ngram rule with logical \texttt{AND} to obtain a logical rule 
%and logical rule provide 
that provides an
accurate boundary of an organization entity \texttt{AdOn GmbH}. 
Although logical rules help us find new entities \emph{explicitly}, rule-based methods usually have high-precision but low-recall results. 
In order to improve the recall of model, we can also find new entities \emph{implicitly} by comparing low-dimensional text representations (i.e.,~word embeddings). 
For example, our rule-based module 
%finds 
might find that
\texttt{Los Angles} is a location entity according to some rules and 
that
\texttt{New York City} has a similar text representation with \texttt{Los Angles} because 
%they are 
both 
are U.S.~cities.
%of the U.S.
%We can easily infer that \texttt{New York City} is also a location entity in the plain text. 
Besides, 
%existing neural NER models are not explainable, 
%but 
readable logical rules can provide convincing explanations for extracted entities 
%so as to alleviate this problem.
to enhance explainability.

Bearing these intuitions in mind, in this paper, we propose a novel weakly supervised named entity recognition (NER) framework, which leverages both a neural NER model and a logical rule-based pseudo label generator to recognize entities \emph{implicitly} and \emph{explicitly}. 
To be specific, our framework starts from only a few seed logical rules (e.g.,~surface form of entities, skip-ngram patterns) given by humans, following which our model will generate all logical rule candidates from templates automatically. 
During training, a neural NER module and rule-based generator will interact with each other iteratively: (1) The rule-based generator can select new logical rules from candidates according to predicted data from a neural NER model; and (2) Meanwhile, rule-labeled data selected by an instance evaluation module will be used for training a re-initialized neural NER model. 
After iterative training, our framework can effectively find new entities from plain text.

%%%%%%%% move to method section
% Specifically, our framework contains three components: (1) A neural NER module, which is a supervised NER model. This module 
% %could
% extracts entities implicitly and is trained by rule-labeled data. In this work, we use a span-based NER model proposed for end-to-end coreference resolution~\cite{Lee2017EndtoendNC}. The span-based framework is flexible because each span is considered as an independent instance. These independent instances make it possible to apply various rules. 
% (2) Weak rule-based label generator. This module includes rule selection and rule labeling. The rule selection is to evaluate all rules and select top rules considering both precision and coverage. We use the patter scoring function from Basilisk~\cite{Thelen2002ABM} as our basic method for evaluation. Rule labeling part is implemented by Snorkel~\cite{Ratner2017SnorkelRT} labeling function. (3) Entity evaluation module. To reduce the noise from the rule-based label generator, we obtain the representation of instances from a pretrained language model and then use local and global scores to evaluate every instance. This module can automatically update thresholds for every entity class according to a high-precision instance set from last iteration.

To 
%our best knowledge, 
the best of our knowledge,
%it is 
our work is
the first 
%time 
to recognize and type entities from only a few rules (e.g.,~20 entities as surface form rules for CoNLL2003 dataset). In summary, our major contributions are:
\begin{itemize}
    \item We conduct NER under a 
    %brand 
    new setting. Compared with previous works using a large dictionary and complicated rules, we 
    %largely reduce 
    %the 
    drastically reduce
    supervision and start from only a few seed rules. Seed rules can be any form from our rule templates (i.e.,~surface form of entities, skip-ngram patterns).
    \item We propose a novel weakly-supervised explainable NER framework. Our framework can automatically generate and select new logical rules according to our rule templates and takes advantage of both explicit rules and implicit word representations to extract entities from plain text. Readable rules also provide explanations for each extracted entity, %largely improve the 
    improving the
    %un
    interpretability of traditional neural models.
    \item We apply our model on three datasets in general and biomedical domains. Our model achieves over \todo{} F1 improvement in three datasets %respectively 
    under 
    %the new 
    our
    setting (i.e.,~a few seed rules). We also conduct a user study in terms of explainability, where results show that our model can explain \todo{} extracted entities.
\end{itemize}


\begin{figure*}[t]
\centering
 %\includegraphics[width=\textwidth]{Figures/Figure2.pdf}
 \includegraphics[width=\textwidth]{Figures/fig-framework-v3.pdf}
\caption{
Overview of our proposed weakly-supervised NER framework by logical rules.
%\hb{Same here, please the share the the link of the slides for this figure}
}
% \vspace{-1mm}
\label{fig:overview}
\end{figure*}

==> 2-related_work.tex <==
%\subsection{Bootstrapping}
%Bootstrapping enables models to obtain large amounts of weakly-labeled data 
Bootstrapping is a technique to learn models
from a small set of seeds, which has been proposed for 
word sense disambiguation \cite{Yarowsky1995UnsupervisedWS} 
and product attribute extraction \cite{putthividhya-hu-2011-bootstrapped}.
%Bootstrapping has also been used for lexicon expansion~\cite{Shen2017SetExpanCS, Yan2019LearningTB} that aims to expand a given lexicon with more semantic members for target semantic classes. 
%which acquires new instances of a specific category by iteratively evaluating and selecting patterns, while extracting and scoring entities. 
\citet{niu2003bootstrapping} applied parsing-based rules in a bootstrapping framework to deal with entity classification.
\citet{Huang2010InducingDS} presented a bootstrapping method to train a semantic class tagger from a small set of seeds. 
To improving scoring in bootstrapping, \citet{Gupta2014ImprovedPL} evaluated pattern scoring based on both seed rules and predicted instances and entity boundaries were determined by part-of-speech tag restriction.
Previous bootstrapping works only focused on assigning semantic labels to pre-extracted phrases without detecting entity boundaries. 
Our work aims to learn a set of logical rules from a small set of seed rules and focuses on detecting entity boundaries and predicting entity labels at the same time. 

%build a NER system from a small set of seed logical rules from 
% ~\cite{Huang2010InducingDS}, which aims to assign a semantic class label for a given phrase candidate without detecting entity boundaries. 
% \citet{Zhang2020BootstrappingNE} leverages dependency parsing rules (i.e.,~``compound'' relations) to recognize entities from text, but dependency parsing rules alone cannot always recognize entities precisely.
% Hence, recognizing entities (i.e.,~boundary information) from plain text is still a challenging task for boostrapping.



%\subsection{Distantly Supervised NER}
Distant supervision~\cite{Mintz2009DistantSF} has been proposed to alleviate human effort by training models using existing lexicons or knowledge bases.
%
% has attracted attention to alleviate human labeling effort. 
%Originally, it was proposed to leverage knowledge bases to supervise relation extraction tasks~\cite{Craven1999ConstructingBK, Mintz2009DistantSF}. 
Recently, there have been attempts to build NER systems with distant supervision~\cite{Ren2015ClusTypeEE, Fries2017SwellSharkAG, Giannakopoulos2017UnsupervisedAT}. 
%
%SwellShark~\cite{Fries2017SwellSharkAG} leverages a generative model to unify and model noise across different supervision sources. However, the heuristic combination of dictionary matching and part-of-speech tag-based regular expressions requires extensive expert effort. %Distant-LSTM-CRF~\cite{Giannakopoulos2017UnsupervisedAT} has been proposed for distantly supervised aspect term extraction, which can be viewed as an entity recognition task of a single type for business reviews. 
AutoNER~\cite{Shang2018LearningNE} trained an NER system by using both typed lexicons and untyped mined phrases as supervision.
%Jiacheng edits:
\citet{Peng2019DistantlySN} proposed an AdaPU algorithm to incorporate an incomplete dictionary as supervision. 
However, lexicons or knowledge bases are not always available for various tasks, especially in specific domains and low-resource settings. 
% All distantly supervised methods rely on an existing knowledge base or dictionary. However, constructing a  %well-performed 
% complete
% dictionary or knowledge base is time-consuming and again might require significant human effort.


%\subsection{Label Generation from Rules}
% Some methods generate labels from heuristic rules. These methods aim at denoising multiple label sources. \citet{Bach2017LearningTS} capture correlations between label sources and dependencies between labels for multiple tasks on the same data~\cite{Bach2019SnorkelDA}. Typically, rule-based methods view a dictionary as one kind of rule.
% \citet{Safranchik2020WeaklySS} proposed a framework for training sequence tagging models with weak supervision consisting of multiple heuristic rules. This method uses tagging rules and linking rules to obtain the position and boundary of an entity respectively. They introduce a generative model to estimate accuracies of the rules and combine their conflicting outputs. The above methods still incur significant costs from rule design and dictionary construction.

Recently, methods have been proposed to obtain weak labels by manually writing labeling functions~\cite{Bach2017LearningTS}.
Based on this idea, several methods~\cite{Safranchik2020WeaklySS,Lison2020NamedER} have been proposed for NER by assuming the availability of a sufficient amount of handcrafted labeling functions and lexicons. 
However, manually designing labeling rules is expensive, and often requires domain expertise.
Our work aims to learn logical rules automatically to reduce human effort. 


% \cite{Lison2020NamedER}




==> 3-formulation.tex <==
Our goal, in this paper, is to extract entities from sentences using, and only using seed logical rules. Each rule consists of the rule body according to our templates and assigned entity type of this rules. Different from previous rule-based methods~\cite{Safranchik2020WeaklySS, Lison2020NamedER} which resort to both rules and a large dictionary, we claim that dictionary for NER systems is also hard to obtain in many cases. Hence, our model only needs a few logical rules given by users to extract entities from plain texts. Please note that logical rules can also be a small dictionary with a few entities.


==> 4-method.tex <==
We introduce our weakly-supervised NER with logical rules framework as follows. First, we present an overview of the whole framework and interactions between modules in Section~\ref{framework}. Then we introduce three components respectively which include a: (1) Logical rule module; (2) Entity evaluation module; and (3) Neural NER module.
%which is a supervised NER model. This module extracts entities implicitly and is trained by rule-labeled data. In this work, we use a span-based NER model proposed for end-to-end coreference resolution~\cite{Lee2017EndtoendNC}. The span-based framework is flexible because each span is considered as an independent instance. These independent instances make it possible to apply various rules. 

%(2) Weak rule-based label generator. This module includes rule selection and rule labeling. The rule selection is to evaluate all rules and select top rules considering both precision and coverage. We use the patter scoring function from Basilisk~\cite{Thelen2002ABM} as our basic method for evaluation. Rule labeling part is implemented by Snorkel~\cite{Ratner2017SnorkelRT} labeling function. 

%(3) Entity evaluation module. To reduce the noise from the rule-based label generator, we obtain the representation of instances from a pretrained language model and then use local and global scores to evaluate every instance. This module can automatically update thresholds for every entity class according to a high-precision instance set from last iteration.

% Our model, \our, contains two parts, span-based neural NER model and rule-based weakly label generator. 
% The two parts interact with each other iteratively and discover the entities in the corpus. Specifically, \our includes the following steps. 
% \begin{itemize}
%     \item Starting from label generator, it applies the rules in rule pool (seeding rules in the beginning) on the training data to obtain weakly labeled data by rules.
%     \item We train a neural NER model on these weakly labeled data from label generator and predict all training data.
%     \item Rule-based label generator automatically infer and select new rules added to rule pool according to the predicted data from NER model. The expanded rule pool will be used for next iteration.
% \end{itemize}
% By repeating the above steps, the performance of our model gets persistent increasing until converges. 
\subsection{Framework Overview}
\label{framework}
In this section, we will introduce entity and rule candidates of our model and then present the interactions between different components. The overview of our framework is illustrated in Figure~\todo{}.

\smallsection{Entity and Rule Candidate Generation}
Our framework enumerates all text spans up to a maximum length in a sentence;
%, but
most of these text spans are not entities. To reduce computational load and provide negative supervision for a neural classifier, we select entity candidates according to noun chunks from the spaCy\footnote{https://spacy.io/} pipeline. All spans of noun chunks and their sub-spans are used as entity candidates.

\textbf{Example 1.} Consider the following sentence:

\texttt{Arafat had decided flying to the West Bank.}

We have \texttt{Arafat} and \texttt{the West Bank} from noun chunks. We use the two text spans and their sub-spans (i.e.,~\texttt{West Bank}, \texttt{the West}, \texttt{Bank}, etc.) as our entity candidates. 

For more accurate entity boundaries, we also use phrases from AutoPhrase~\cite{Shang2018AutomatedPM} to group sub-spans together. For instance, if we obtain the phrase \texttt{West Bank} in Example 1, spans \texttt{West Bank}, \texttt{West} and \texttt{Bank} are considered as one candidate in the following rule matching. Any sub-span (e.g.,~\texttt{Bank}) is selected by rules, then \texttt{West Bank} is considered as a rule-matched entity.

Rule candidates are generated from entity candidates according to our rule templates. Given entity candidate \texttt{West Bank} and logical rule template \texttt{PreNgram} $\land$ \texttt{POStag} introduced in Section~\ref{rule}, we obtain rule candidate ``flying to the $\land$ PROPN, PROPN''. We generate all entity and rule candidates before iterations.

\smallsection{Interactions between Modules}
The predicted data from the neural NER module provides an instance set to evaluate and select logical rule candidates. In practice, $\sigma$ (empirically $70$) percent
%age 
of the most confident predicted data is sent to the logical rule module. Meanwhile, rule labeled data will be used as a training set for the neural NER module training in the next iteration. To reduce the semantic drift caused by rules, we adopt an entity evaluation module introduced in Section~\ref{eval module}. All rule-labeled data will be scored and selected before being used as training data.

After iterations, we use the output of the trained neural NER module as the final entity
%ies 
prediction results.

\subsection{Logical Rule Module}
\label{rule}
In this section, we introduce a logical rule module including rule templates (i.e.,~atomic rules and logical rules) and a rule selection strategy. The rule module 
%could 
can
select new rules from rule candidates generated from 
the
corpus and apply rules on all unlabeled text spans. 

\smallsection{Atomic Rules}. 
The
atomic rule $r_{t_i}$ 
is 
the atomic matching logic generated from rule template $t_i$. Every atomic rule has its own label. In our model, we design five atomic rule templates for NER shown as follows: (1) \texttt{SurfaceForm}: Surface name matching with given full name of entities. (2) \texttt{PreNgram}: Match the previous $N$ words before the entities. (3) \texttt{PostNgram}: Match the posterior $N$ words after entities. (4) \texttt{POStag}: Match part-of-speech patterns of entities. (5) \texttt{PreDependency}: The parent node and sibling nodes of entities on the dependency tree.
% \begin{itemize}
%     \item \textbf{SurfaceForm}. Surface name matching with given full name of entities.
%     \item \textbf{Prefix}. Match the prefix of span with rules.
%     \item \textbf{Suffix}. Match the suffix of span with rules.
%     \item \textbf{PreNgram}. Match the previous contextual texts.
%     \item \textbf{PostNgram}. Match contextual texts after span.
%     \item \textbf{POStag}. Match part-of-speech pattern with rules.
%     \item \textbf{PreDependency.} The parent and siblings of the span on the dependency tree.
% \end{itemize}
\todo{ Add detailed descriptions about these 5 types of rules in Appendix}

\textbf{Example 2.} Consider the following sentence, the entity in this sentence is \texttt{AdOn GmbH}.

\texttt{The new company is called AdOn GmbH and is located in Hamburg.}

If we have a \texttt{PreNgram} rule `company is called \{*\}', we will match the following spans: [\texttt{AdOn}], [\texttt{AdOn GmbH}], [\texttt{AdOn GmbH and}], etc.~until up to the max span length 
%of span 
we set. 

We can see from the above example, other than SurfaceForm, atomic rule
methods 
will introduce 
%lots of 
noisy spans. 
%So 
As such,
atomic rules cannot identify an entity individually. 

\smallsection{Logical Rules}
To obtain a precise entity in a sentence by rules, we need to compose different atomic rules to get accurate entity boundary information. Therefore, we propose composing atomic rules into logical rules. Logical rules are the composition of atomic rules by logical conjunction $\land$. Formulated as:
\begin{equation}
    \textbf{r}_{composed} = r_1 \land r_2 \land \ldots \land r_n
\end{equation}
where $r_1, r_2,\ldots,r_n$ are atomic rules.

\textbf{Example 3.} A simple example of a  logical rule. The following sentence has entity \texttt{AdOn GmbH}.

\texttt{The new company is called AdOn GmbH and is located in Hamburg.}

If we have a logical rule $r_1 \land r_2$ from template \texttt{PreNgram} $\land$ \texttt{POStag}, where $r_1$ is `company is called \{*\}' and $r_2$ is `PROPN PROPN', we will exactly match with the entity \texttt{AdOn GmbH}.

In our model, we use logical conjunction with two atomic rules to get a logical rules

\smallsection{Rule Selection Strategy}
Every iteration, our logical rule module selects new rules from candidates based on rule scores. All text spans predicted by the NER model will be used for rule evaluation. Spans that are predicted as typed entities are called category members for rule selection.  We adopt the method from Basilisk~\cite{Thelen2002ABM} to calculate the score for rule $r_i$:
\begin{equation}
    F(r_i) = \frac{F_i}{N_i} \log_2(F_i)
\end{equation}
where $F_i$ is the number of category members extracted by rule $r_i$ and $N_i$ is the total number of spans extracted by rule $r_i$. Intuitively, this method considers both the precision and recall of rules because 
%the
$\frac{F_i}{N_i}$ is the precision 
%score 
of the rule and $\log_2(F_i)$ represents the rule's ability to cover more spans. For example, $r_1$ could match 100 instances ($N_1=100$) and 80 of them are category members ($F_1=80$), so the score $F(r_1) = \frac{80}{100}\log_2(80) \approx 5.06$.

For each category of entities, the top $\mathrm{K}$ rules are selected for labeling data. Our model uses a value of $\mathrm{K}=20$ for the first iteration. To prevent low-precision rules, we also set a threshold $\tau$ to $0.9$ for precision of rules. This method allows a variety of logical rules to be considered, yet is precise enough that all logical rules are strongly associated with the category. 

\subsection{Entity Evaluation Module}
\label{eval module}
To alleviate semantic drift and error propagation in iterative framework, in this module, we evaluate every rule labeled entity by local and global scores introduced in entity set expansion~\cite{Zhang2020EmpowerES}. We maintain a high precision entity set. Such a set is initialized with entities matched with seed rules and expanded with the selected entities. The expanded set will be used for evaluation in the next iteration. With a high precision set, we can dynamically compute selection thresholds for each category in each iteration. 
%Dynamic thresholds will be used for rule labeled selection.

\smallsection{Local and Global Scores}
Given a high precision entity set $H_i$ belonging to category $i$ and a query entity instance $e_q$, we use the averaged first three layers outputs of a pre-trained language model (e.g.,~BERT~\cite{Devlin2019BERTPO}, SciBERT~\cite{Beltagy2019SciBERTAP}) to encode the whole sentence and extract tokens in an entity. The average token representation in an entity is the contextual representation $\mathbf{x}_e$ of the entity $e_i$ belonging to category $i$. The first three layers' outputs include more word-level information which represents entities better without fine-tuning. We also compute representations for entities in the high precision set in the same way.

The local score between the query entity and the entity set is calculated as:
\begin{equation}
    \mathrm{score}^{\mathit{loc}}_{i} = \max_{e_i\in H_i} \mathbf{\cos}(\mathbf{x}_{e_i}, \mathbf{x}_{e_q})
\end{equation}
where $\mathbf{\cos}(\mathbf{x}_{e_i}, \mathbf{x}_{e_q})$ is the cosine similarity between 
vectors 
$\mathbf{x}_{e_i}$ and $\mathbf{x}_{e_q}$. $\max$ finds the maximum similarity between entities in $H_i$ and query entity $e_q$.
Local scores help to find new entities but 
%it is more 
can
easily introduce noise into the high precision set $H_i$. Therefore, to measure similarity between query entities and target categories better, we introduce the global score. 

Given the high precision set $H_i$, we sample a small set $E_s$ (typically of size 3) and use the average $\mathbf{x}_{E_s}$ of all entity representations to represent $E_s$. We repeat the above step $N$ times. Then, the global score is calculated as:
\begin{align}
    \mathrm{score}^{\mathit{glb}}_{i}&= \frac{1}{N}\sum_{1\leq j\leq N} \mathbf{\cos}(\mathbf{x}^{j}_{E_s}, \mathbf{x}_{e_q})\\
    \mathbf{x}^{j}_{E_s} &= \frac{1}{|E_s|}\sum_{x_e\in E_s} \mathbf{x}_e
\end{align}
In our experiments, $N=50$ and $E_s$ is usually a small set (otherwise, the average representation of a large set would reduce information). Such a global score complements the above local score and we use 
%their 
the
geometric mean to 
finally obtain
scores of all query entities:
\begin{equation}
    \label{score}
    \mathrm{score}_{i} = \sqrt{\mathrm{score}^{\mathit{loc}}_{i} \times \mathrm{score}^{\mathit{glb}}_{i}}
\end{equation}

\smallsection{Dynamic Threshold}
Different kinds of entities usually different similarity with each other in pre-trained language models. High-frequency entities (e.g.,~locations) are more similar to each other than low-frequency entities (e.g.,~person names). Moreover, there is a 
%big 
difference in terms of 
the
number of entities rules can match. Therefore, selection methods based on fixed top-$k$ or a fixed threshold for every iteration are not 
%reasonable. 
ideal.
To deal with the above problem, we use a dynamic threshold which is calculated according to a high precision entity set.
To be specific, we hold out one entity instance 
%out 
in the high precision set and compute the evaluation score from Eq.~\ref{score}. We repeat $T$ times to obtain the minimum value. The threshold for category $i$ is calculated as:
\begin{equation}
    \mathrm{threshold} = \tau \cdot \min_{k\leq T, e_k \in H_i} \mathrm{score}_i (e_k)
\end{equation}
where $e_k$ is the held out entity instance and $\tau \in [0, 1]$ is a temperature to control the final threshold. When $\tau =0$ 
%means 
we select all new entities; 
%$\tau=0.8$ is identical in all our experiments.
we set $\tau=0.8$ in all our experiments.

\subsection{Neural NER Module}

In this section, we introduce the neural NER module in our model. Traditional named entity recognizers follow the sequence labeling framework using \texttt{IOB} or \texttt{IOBES} schemes~\cite{Ratinov2009DesignCA}. However, sequence labeling is not suitable for rule-based labeling because tokens' labels rely on 
%its 
contextual text. For flexibility, we follow
a
span-based information extraction (IE) framework first designed for end-to-end coreference resolution~\cite{Lee2017EndtoendNC}
%and then span-based framework was 
which has been
adapted for other tasks~\cite{Luan2019AGF, Jiang2020GeneralizingNL, Wadden2019EntityRA, He2018JointlyPP, Dixit2019SpanLevelMF}. In this framework, all possible spans are enumerated 
%and predicted to determine 
to predict whether
%if 
they are entities. Due to its flexibility, we can consider each span as an independent instance when applying rules to it.

\smallsection{Span Representation} Given a sentence $\mathbf{x} = [w_1, w_2,\ldots,w_n]$ of $n$ tokens, a span $s_i = [w_{b_i}, w_{b_{i+1}}, \ldots, w_{e_i}]$, where $b_i, e_i$ are the start and end indices respectively. The representation of spans contains two components: a content representation $\mathbf{z}_i^c$ calculated as the weighted average across all token embeddings in the span, and a \textit{boundary representation} $\mathbf{z}_i^u$ that concatenates the embeddings at the start and end positions of the span. Specifically,
\begin{equation*}
    \begin{aligned}
	\mathbf{c}_1, \mathbf{c}_2, \ldots, \mathbf{c}_n &= \mathrm{TokenRepr}(w_1, w_2, \ldots, w_n),\\
	\mathbf{u}_1, \mathbf{u}_2, ..., \mathbf{u}_n &=  \mathrm{BiLSTM}(\mathbf{c}_1, \mathbf{c}_2,\ldots,\mathbf{c}_n),\\
	\mathbf{z}_i^c &= \mathrm{SelfAttn}(\mathbf{c}_{b_i}, \mathbf{c}_{b_i+1}, \ldots, \mathbf{c}_{e_i}),\\
	\mathbf{z}_i^u &= [\mathbf{u}_{b_i}; \mathbf{u}_{e_i}], \mathbf{z}_i = [\mathbf{z}_i^c;\mathbf{z}_i^u],
\end{aligned}
\end{equation*}
where $\mathrm{TokenRepr}$ could be non-contextualized, such as Glove~\cite{Pennington2014GloveGV}, or contextualized, such as BERT~\cite{Devlin2019BERTPO}. $\mathrm{BiLSTM}$ is a bi-directional LSTM layer and $\mathrm{SelfAttn}$ is a self-attention layer. For further details please refer to \citet{Lee2017EndtoendNC}.

\smallsection{Span Prediction} We predict labels for \textit{all} spans up to a fixed length of $l$ words using a multilayer perceptron (MLP):
\begin{equation}
    \mathbf{o}_i = \mathrm{softmax}(\mathbf{MLP}^{\mathrm{span}}(\mathbf{z}_i))
\end{equation}
where $\mathbf{o}_i$ is prediction for the span. We introduce one negative label \texttt{NEG} as an additional label which indicates invalid spans (i.e.,~spans that are not named entities in the corpus).

% \subsection{Interaction between NER Model and Rule-based Label Generator}


% Specifically, rule-based label generator applies labeling rules on unlabeled data to get weakly labeled data. These data usually only cover a small part of whole dataset, because we have limited seeding rules at the beginning. We train a neural NER model on these weakly labeled data. Because neural NER model is based on implicit representation, it will predict new entities as category member which are similar with the existing labeled data in terms of semantic distance. For instance, we have seeding rule `Lon* -> LOC’ which means if prefix of span is `Lon’, then the span is a location, so all spans ‘London’ will be labeled a location. After getting these sentences, NER model is trained on them and makes prediction on whole dataset.  The span `Singapore’ is very likely predicted as a location entity, because `Singapore’ and ‘London’ have the very closed distance in implicit semantic representation. With these new entities predicted by NER model, rule-based label generator will evaluate and select more rules to add to the rule pool. The next iteration will begin with the expanded rule pool.



==> 5-experiments.tex <==
%\hb{Please add results in tables}
% \todo{.

% Jiacheng, please add some items here, to briefly mention what experiments need to do before submission. 

% ** rule labler results *

% * weakly supervised method https://www.aclweb.org/anthology/2020.acl-main.139.pdf


% ** Performance with Different Number of Seeds.

% ** Different Strategy of Selecting Rules.

% }


\begin{table*}[h]
    \center
    % \vspace{-2mm}
%\scalebox{0.87}{
    \small
    \begin{tabular}{r|ccc|ccc|ccc}
        \toprule
                & \multicolumn{3}{c}{BC5CDR}  & \multicolumn{3}{c}{CHEMDNER} & \multicolumn{3}{c}{CONLL2003}\\
                    
        \cmidrule{2-10}
        Methods     &  Precision & Recall & F$_1$ & Precision & Recall & F$_1$ &  Precision & Recall & F$_1$ \\
        \midrule
        Seed Rules & 94.09 & 3.81 & 7.33 & 91.60 & 13.19 & 23.07 & 95.77 & 2.76 & 5.36\\
        
        LinkedHMM & 10.18 & 15.60 & 12.32 & 23.99 & 10.77 & 14.86 & 19.78 & 31.51 & 24.30\\
        
        HMM-agg. & 43.70 & 21.60 & 29.00 & 49.60 & 18.40 & 26.80 & 52.00 & 8.50 & 14.60\\
        
        CGExpan & 40.96 & 24.75 & 30.86 & 45.70 & 25.58 & 32.80 & 55.97 & 28.7 & 37.95\\
        
        AutoNER & 42.22 & 30.66 & 35.52 & 66.83 & 27.59 & 39.05 & 32.07 & 5.98 & 10.08 \\ 
        
        Seed Rule + Neural NER & 78.33 & 21.60 & 33.86 & 84.18 & 21.91 & 34.78 & 72.57 & 24.68 & 36.83\\
        
        Self-training & 73.69 & 29.55 & 42.19 & 85.06 & 20.03 & 32.42 & 72.80 & 24.83 & 37.03\\  
        
        \midrule
        Learned Rules Only & 79.29 & 18.46 & 29.94 & 69.86 & 21.97 & 33.43 & 65.51 & 21.12 & 31.94\\
        Ours w/o Autophrase   & 74.56 & 32.93 & 45.68 & 67.74 & 55.99 & 61.31 & 71.37 & 25.50 & 37.57\\  
        Ours w/o Instance Selection& 58.7 & 63.37 & 60.95 & 42.64 & 48.25 & 45.27 & 58.51 & 58.8 & 58.65\\
        Ours & 66.53 & {\bf 66.94} & {\bf 66.73} & 63.01 & {\bf 60.18} & {\bf 61.56} & 64.29 & {\bf 64.14} & {\bf 64.22}\\  
        \bottomrule
    \end{tabular}
    \caption{
    Precision, recall, and micro-average F1 of baselines and our methods.
    }
    \label{tab:main_perf}
%}
    % \vspace{-1mm}
    \end{table*}

In this section, we empirically evaluate our weakly-supervised NER model and 
%compared models 
others
on real-world datasets. We first introduce the datasets and experimental settings. Then, we present NER performance and some case studies about iterations, seeds and rule selections. Finally, we conduct a user study about explainable NER.
\hb{this needs to be condensed, just briefly mention what's in the experiment section. }

\subsection{Experimental Setting}
\hb{dataset part, can be further condensed, Need to emphasize that we did not use any labels from training set. }

\smallsection{Datasets}
We consider data for three biomedical and general tasks:
\begin{itemize}
    \item \textbf{BC5CDR}~\cite{Li2016BioCreativeVC} is the BioCreative V CDR task corpus. It contains 500 train, 500 development, and 500 test PubMed articles, with 15,953 chemical mentions and 13,318 disease mentions.
    \item \textbf{CHEMDNER}~\cite{Krallinger2015TheCC} is a collection of 10,000 PubMed abstracts that contain a total of 84,355 chemical entity mentions labeled manually by experts. After filtering out sentences with chemical entities, there are 
    %$14,522$/$14,572$/$12,434$
    14,522/14,572/12,434
    sentences in training/development/test datasets respectively.
    \item \textbf{CoNLL2003}~\cite{Sang2003IntroductionTT} consisting of 14,041/3,250/3,453 sentences in the training/development/test set extracted from Reuters news articles. We only include \texttt{PERSON}, \texttt{LOCATION} and \texttt{ORGANIZATION} entities in our experiments, because there are several types of entities in the \texttt{MISC} category and a few seeds cannot cover all types.
\end{itemize}

\smallsection{Metrics}
We use the micro-averaged $F_1$ score as the 
main 
evaluation metric,
%. Meanwhile, 
and also report
precision and recall.
%are presented. 
All 
models 
%reported 
are trained on the training set, 
%tune 
hyperparameters 
are tuned
on 
the
development set,
%and report the performance on test dataset.
and performance is reported on the test set.
\hb{this part can be removed! in the details part, we already said that we tune on dev. }

\smallsection{Parameters and Model Training}
In our neural NER module, we conduct optimization with an Adam optimizer with learning rate $2e^{-5}$. We use a batch size of $32$ for all experiments. A dropout 
%of a 
ratio $0.5$ is applied. For better stability, we use gradient clipping of $5.0$. Maximum length of spans is $5$.
In our logical rule module, we select the top $20$ rules every iteration for each entity category for BC5CDR, CoNLL2003 dataset, and $60$ rules for the CHEMDNER dataset. Precision thresholds for rules are 0.9 for all experiments. In the entity evaluation module, the temperature of thresholds is $0.8$. The pre-trained language models are SciBert for two biomedical datasets and Bert for CoNLL2003 dataset. During training, we 
%iterate 
run
the framework 
for
$32$ 
%times 
iterations
for all datasets and 
%apply 
select
the best model on the development set.
%for final test.
\hb{Yes, most of the details can be moved to Appendix, maybe keep max-length of 5, and 20 seed rules. }

\smallsection{Seed Rule Selection}
Due to high precision, we use \texttt{SurfaceForm} as seed logical rules for all experiments. To be specific, we manually select $20$ high-frequency entities in total as seed rules for BC5CDR and CoNLL2003 and $40$ entities for CHEMDNER because of its
%a 
large 
%amount 
number
of entities. We
%will 
compare our model starting with different seed rules in Section~\ref{diff seed}.
\hb{needs to rephrase a little, to be more clear. }
\todo{Needs to add seed rules for each dataset in the Appendix section}

\subsection{Comparison Methods}
\hb{May need to condense the descriptions of each baseline}

\noindent\textbf{Seed rule matching}. We apply seed rules to the test set directly to obtain entity mentions with exactly the same surface name as the seed rules.

\noindent\textbf{CGExpan}~\cite{Zhang2020EmpowerES} is a state-of-the-art entity set expansion method by probing a language model. 
%In our experiments, we use SciBert~\cite{Beltagy2019SciBERTAP} as a language model for BC5CDR and CHEMDNER and the original BERT for CoNLL2003.
In our experiments, we use BERT  as a language model for CoNLL2003 and SciBert~\cite{Beltagy2019SciBERTAP} for BC5CDR and CHEMDNER.
For every dataset, we select $200$, $500$, $800$, $1000$ as our target expanded size to get an expanded entity set. Then, we apply the expanded entity set on the test set by surface name matching.

\noindent\textbf{AutoNER}~\cite{Shang2018LearningNE} takes dictionaries of typed terms and untyped mined phrases as input. We apply the best expanded entity set from CGExpan as typed terms. The expanded entity set and mined phrases from AutoPhrase~\cite{Shang2018AutomatedPM} are used as untyped mined phrases.

\noindent\textbf{LinkedHMM}~\cite{Safranchik2020WeaklySS} introduces a new type of generative model to incorporate noisy rules as supervision. In our experiments, we view expanded entity sets as tagging rules and mined phrases as linking rules and use the neural NER model as the final result.

\noindent\textbf{HMM-agg.}~\cite{Lison2020NamedER} 
%replies on 
applies
a broad spectrum of labelling functions to automatically annotate text from the target domain. A hidden Markov model merges these annotations and a sequence labelling model is finally trained on aggregated annotations. We use our expanded entity set as gazetteers labeling functions in this model and results from sequence labelling model as final results.

\noindent\textbf{Seed Rule + Neural NER}. This method is our framework without iteration. After rule labeling with seed rules, we use rule-labeled data as supervision to train a span-based neural NER model and use the result of the NER model as our final result.

\noindent\textbf{Self-training}. This method is our framework without the logical rule module and instance selection module. We use the results from the neural NER model as a training set for the next iteration.

\hb{Very wired to put ablation methods with baselines, may need to re-organize little....}
\noindent\textbf{Ablation version}. We also test our framework without mined phrases from Autophrase and 
%framework 
without our instance evaluation module.

\noindent\textbf{Rule Module}. We apply learned logical rule learning from the training set and report the logical rule performance on the test set.

All implementations of compared methods are from author-provided Github repositories,
%. We tried our best to tuning hyper-parameters and 
with hyper-parameters tuned
following authors' experimental settings.

\subsection{NER Performance Comparison}
\hb{Too long..., may just need half column to tell reviewers, what are important, too much info will confuse reviewers, dilute the effectiveness of our method}

We present F$_1$, precision, and recall scores on all datasets in Table~\ref{tab:main_perf}. We 
%can 
find that our framework achieves the best performance when 
%only 
given only a few seed entities as supervision. 

CGExpan can expand new entities in the same categories but 
%meanwhile 
introduces 
%some 
errors into the expanded entity set. We find that CGExpan suffers from semantic drift on low frequency entities.
%when entities are low frequency. 
For example, CGExpan cannot
%tell
detect
\texttt{ORG} and \texttt{PER} 
%well 
effectively
in the CoNLL2003 dataset.

Existing weakly supervised methods (i.e.,~AutoNER, LinkedHMM and HMM-agg.) cannot recognize entities 
%well 
effectively
under such weak supervision. 
%Their 
Such
methods usually require high-precision dictionary matching as supervision. However, our high-precision seed rules cannot provide enough coverage while
the
expanded entity set from CGExpan cannot provide 
%precision 
precise
enough supervision. 
%Their 
These
supervised modules can even produce worse performance than string matching when supervision is very noisy. For example, LinkedHMM has worse results than CGExpan on both the BC5CDR and CHEMDNER datasets because supervision from CGExpan is noisy (i.e.,~precision is low). But if we only use seed rules, a large amount of supervision are false negative for their training which usually leads to worse results.

Our framework without iteration (i.e.,~Seed Rules + Neural NER) and self-training can achieve high-precision results because our framework provides a large amount of entity candidates during training. These entity candidates will not be used for parameter updates until they are labeled as entities or negative. However, these two methods are hard to find new entities from corpus.

We also design two ablations
%versions 
of our framework. The framework without Autophrase results usually does not have enough entity candidates at the beginning, which undermines the ability to 
%recognizing 
recognie
new entities. Hence, from Table~\ref{tab:main_perf}, the framework without Autophrase has high precision but low recall.
%results. 
Another ablation 
%version 
is to remove our entity evaluation module. 
The
framework without entity evaluation has lower precision 
%results 
than the original. Such results indicate the effectiveness of the entity evaluation module.

\begin{figure*}[t]
     \centering
     \begin{subfigure}{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/bc5cdr_iter_f1.png}
         \caption{BC5CDR}
         \label{fig:bc5cdr_iter_f1}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/chemdner_iter_f1.png}
         \caption{CHEMDNER}
         \label{fig:chemdner_iter_f1}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/conll_iter_f1.png}
         \caption{CoNLL2003}
         \label{fig:conll_iter_f1}
     \end{subfigure}
    \caption{Iterations vs.~Performance of the neural NER module on three datasets.}
    \label{fig:iter_f1}
\end{figure*}

%\subsection{Case Study of Performance}
\subsection{Performance Case Study}

\smallsection{Performance vs.~Iterations}
Figure~\ref{fig:iter_f1} demonstrates the performance of 
the 
neural NER module 
%over iterations 
as we iterate
on three datasets. We can see that 
the
performance of 
the
neural NER module 
%are 
consistently 
%improved 
improves
on all three datasets 
%with iterations. 
as we iterate.
Our framework converges at the 
%$25_{th}$ 
$25^{\text{th}}$
iteration and maintains a stable $F_1$ 
score 
after convergence. Figure~\ref{fig:iter_f1} indicates that our framework can effectively find new entities starting from a few seed rules in different domains.

\hb{Maybe we could combine Figure 3 and 5, to save space}

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{Figures/diff_seeds.png}
    \caption{
    %The 
    Performance with different seed rules on three datasets.
    }
    \label{fig:diff_seed}
\end{figure}

\smallsection{Performance with Different Numbers of Seeds}
\label{diff seed}
We conduct 
%our 
experiments starting from different numbers of seed rules on three datasets. Figure~\ref{fig:diff_seed} presents 
%F$_1$ 
$F_1$
%score 
scores
under different seed settings. We can see that:
For BC5CDR and the CoNLL2003 dataset, 20 seed entity can provide enough supervision to achieve performance about $65$ F$_1$. This indicates 
%that 
the effectiveness of our framework under extremely weak 
%supervisions.
supervision.
The performance increases or drops slightly if we continue adding more seed entities for BC5CDR and the CoNLL2003 dataset. One reason is that our model has detected most entities that can be matched by rules. More seeds 
cannot 
bring more coverage of entities.
The 
CHEMDNER dataset contains more sentences than the other two datasets, so adding more seeds 
%can 
achieves consistent performance increases.
%of performance.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.49\textwidth]{Figures/compare_autoner.png}
    \caption{
    F1 comparison between different sizes of dictionary for AutoNER and our model on BC5CDR dataset.
    }
    \label{fig:compare_distant}
\end{figure}

\smallsection{Comparison with Distant Supervision}
To demonstrate the effectiveness of our logical rule module, we try to compare our method with distant supervision from 
a
knowledge base.

Specifically, we conduct experiments on the BC5CDR dataset by sampling different amounts
of entities in 
a
dictionary for AutoNER training. We also include the 20 seed entities in our experiments. As shown in Figure~\ref{fig:compare_distant}, when the size of
the
dictionary is $0$, we use only the $20$ seed entities as typed terms and untyped phrases for AutoNER. Then every time we sample $500$ typed terms and add them into the dictionary for AutoNER. To achieve similar 
%F$_1$ 
$F_1$
score (i.e.,~66.73\%) with our framework, AutoNER needs more than $2,000$ distantly supervised entities. Such results indicate the effectiveness and usefulness of our framework in the scenario without an existing knowledge base as distant supervision.

\begin{table}[t]
    \center
    \small
    \begin{tabular}{r|ccc}
        \toprule
        Strategy & Precision & Recall & $F_1$\\      
        \midrule
         Rule Type & 57.14 & 63.00 & 59.93\\
         Entity\&Rule Type & 61.73 & 64.97 & 63.31\\
         Entity Type & \textbf{66.53} & \textbf{66.94} & \textbf{66.73}\\
        \bottomrule
    \end{tabular}
    \caption{Performance on the BC5CDR dataset with three different rule selection strategies.
    }
    \label{tab:strategies}
\end{table}
%\smallsection{Different Strategies of Rule Selection}
\smallsection{Rule Selection Strategies}
To compare different strategies 
%of
for
selecting logical rules, we conduct experiments with three different strategies on 
the
BC5CDR dataset: (1) Top $\mathrm{K}$ rules for each entity category. (2) Top $\mathrm{K}$ rules for each logical rule type. (3) Top $\mathrm{K}$ rules for each entity and logical rule type.

As shown in Table~\ref{tab:strategies}, our framework achieves the best performance when we select
the
top $\mathrm{K}$ rules for each entity during every iteration. The results of different strategies have similar recall but different precision which means we select some wrong rules during iterations. Such results indicate that our dataset usually has balanced entity types instead of balanced rule types. Hence, if we select
the
same number of rules for each rule type, we will introduce some wrong rules. Our precision threshold $\tau$ can alleviate this problem but we prefer selecting same number of rules for each entity type.

\subsection{Case Study of Logical Rules}
\begin{table}[t]
    \center
    
    \small
    \begin{tabular}{r|ccc}
        \toprule
        Rule type &  BC5CDR &  CHEMDNER &  CoNLL2003 \\
        \midrule
         Surface & 503 (41\%) & 1667 (44\%) & 779 (25\%)\\
         Pre+Post & 203 (17\%) & 629 (17\%) & 956 (31\%)\\
         Pre+POS & 288 (24\%) & 585 (16\%) & 455 (15\%)\\
         POS+Post & 149 (12\%) & 418 (11\%) & 438 (14\%) \\
         Dep+POS & 79 (6\%) & 432 (12\%) & 469 (15\%) \\
        \bottomrule
    \end{tabular}
    \caption{Number and ratio of different logical rule types on all datasets.}
    \label{tab:num_rules}
\end{table}

% * how many test cases can be matched by the learned rules 

% * in these matched cases, how many are correct and incorrect?
\smallsection{Number of Learned Logical Rules}

Table~\ref{tab:num_rules} provides 
%the
numbers and ratios of different logical rules learned during all iterations. We can see that \texttt{SurfaceForm} works 
critically 
in BC5CDR and CHEMDNER dataset, which indicates the importance of traditional lexicon-based bootsrapping for NER tasks. CoNLL2003 has more 
%logical rule 
\texttt{PreNgram}+\texttt{PostNgram}
logical rules, which means we can easily find entities from
%its 
contextual information.

When we apply learned logical rules on 
the
test set of BC5CDR, 
%there are 
$2,556$ entity instances are matched with logical rules. Among them, $1,898$ instances are predicted by rules correctly and $658$
%instances 
are incorrect.

\begin{table*}[t]
    \center
    
    
    \small
    \begin{tabular}{p{9cm}p{6cm}}
        \toprule
        Sentences & Logical rules \\
        \midrule
        This occlusion occurred after EACA therapy in a patient with {\color{red}SAH} and histopathological documentation of recurrent SAH. 
        & PreNgram: a patient with
        $\land$ PostNgram: and\\
       
        We also analyzed published and unpublished follow-up data to determine the risk of {\color{red}ICH} in antithrombotic users with MB.
        & PreNgram: the risk of $\land$ POStag: PROPN\\
        
        3 weeks after initiation of amiodarone therapy for {\color{red}atrial fibrillation}.
        & PreNgram: therapy for $\land$ POStag: ADJ NOUN\\
        
        Although 25 mg of {\color{red}lamivudine} was slightly less effective than 100mg (P=.011) and 300 mg ( P=.005).
        & PreNgram: mg of $\land$ POStag: NOUN\\
        
        These results suggest that the renal protective effects of {\color{red}misoprostol} is dose - dependent.
        & PreNgram: protective effect of $\land$ POStag: NOUN\\
        \bottomrule
    \end{tabular}
    \caption{Examples of sentences and matched rules in 
    the
    BC5CDR test set. Rule-matched entities are highlighted in red.}
    \label{tab:rule_example}
\end{table*}



\smallsection{Explanations 
%Provided by 
from
Logical Rules}

\hb{Please add some stats about how many instances can be matched by our learned logical rules}
\hb{add how many of the matched are correct}
\hb{how many of these matched cases can be explained?}


Logical rules not only rapidly find new entities in the corpus, but provide explanations for NER results. Table~\ref{tab:rule_example} represents some examples of sentences and learned logical rules in the test set of BC5CDR. We can see that logical rules provide convincing explanations. For example, we could easily infer that ``therapy for'' followed by a ``ADJ NOUN'' and the ``ADJ NOUN'' is a disease. Compound logical rules provide accurate type and boundary information for recognized entities.

%For further exploring if 
To further explore whether
logical rules can provide explanations for NER results, we design a user study. In the study, we sample $100$ sentences matched with at least one logical rule 
other than SurfaceForm and let two users and two biological experts to annotate whether our learned logical rules can explain recognized entities well in 
the
BC5CDR dataset. 

% * For incorrect cases, analyze reasons 

% * analysis of not-matched cases..
\begin{table*}[t]
    \center
    
    \small
    \begin{tabular}{lcc}
        \toprule
        Text & Ground truth & Error type \\
        \midrule
        Early postoperative {\color{red}delirium} incidence risk... & postoperative delirium & nested entity \\
        ...the risk of {\color{red}drug} - induced hepatic injury... & Negative &  general meaning\\
        ...call attention to the risk of {\color{red}tacrolimus} use in patients... & Negative & semantic drift\\
        ...induced {\color{red}disturbed cholesterol homeostasis} was studied. & cholesterol & inaccurate boundary \\
        \bottomrule
    \end{tabular}
    \caption{Common error instances and error types on 
    the
    BC5CDR dataset. Rule-matched entities are highlighted 
    %with 
    in
    red.}
    \label{tab:error_example}
\end{table*}


\smallsection{Error Analysis of Rules}

\hb{It's better to add some stats about the percentage of each type of errors, which can be estimated by the samples you manually checked}

We analyze the NER results from the BC5CDR dataset and conclude the following common error 
%reasons 
conditions as
shown 
%as 
in
Table~\ref{tab:error_example}:

%
(1) When entities include another entity, \texttt{SurfaceForm} rules are likely to match the shorter one.

(2) Some words (e.g.~location, drug) express general meaning 
%but 
that
our rules cannot identify.

(3) Although our entity evaluation module largely alleviates
%the 
semantic drift, 
%there still exists some cases.
it still occurs in some cases.

(4) Logical rules provide accurate boundary information in most cases, but still cannot identify entities in a phrase.


% \begin{figure*}[t]
%      \centering
%      \begin{subfigure}{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/BC5CDR_Rule_Pie.png}
%          \caption{BC5CDR}
%          \label{fig:bc5cdr_rules}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/CHEMDNER_Rule_Pie.png}
%          \caption{CHEMDNER}
%          \label{fig:chemdner_rules}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/CoNLL2003_Rule_Pie.png}
%          \caption{CoNLL2003}
%          \label{fig:conll_rules}
%      \end{subfigure}
%         \caption{Numbers of selected logical rules.}
%         \label{fig:rules}
% \end{figure*}


